Augmenting Policy Learning with Routines Discovered from a Single Demonstration

Humans can abstract prior knowledge from very little data and use it to boost skill learning. In this paper, we propose routine-augmented policy learning (RAPL), which discovers routines composed of primitive actions from a single demonstration and uses discovered routines to augment policy learning. To discover routines from the demonstration, we first abstract routine candidates by identifying grammar over the demonstrated action trajectory. Then, the best routines measured by length and frequency are selected to form a routine library. We propose to learn policy simultaneously at primitive-level and routine-level with discovered routines, leveraging the temporal structure of routines. Our approach enables imitating expert behavior at multiple temporal scales for imitation learning and promotes reinforcement learning exploration. Extensive experiments on Atari games demonstrate that RAPL improves the state-of-the-art imitation learning method SQIL and reinforcement learning method A2C. Further, we show that discovered routines can generalize to unseen levels and difficulties on the CoinRun benchmark.

==> text/s0_Algorithm_detail.tex <==
% MDP process
\newcommand{\MDP}{\Gamma}
\newcommand{\MDPS}{\mathcal{S}}
\newcommand{\MDPA}{\mathcal{A}}
\newcommand{\MDPT}{\mathcal{T}}
\newcommand{\MDPR}{\mathcal{R}}
\newcommand{\MDPDIS}{\gamma}
\newcommand{\MDPPOLICY}{\pi}
% Routines
\newcommand{\MRDPL}{\mathcal{L}}
\newcommand{\MixedAction}{ \widetilde{\rho}}
\newcommand{\LengthRt}{ {\left|\rho \right|}}
\newcommand{\LengthMixed}{ {\left|\widetilde{\rho}\right|}}
\newcommand{\AugmentedActionSpace}{\widetilde{\mathcal{L}}}

\begin{algorithm}[htb]
  \caption{RoutineDiscovery}
  \label{alg:routine_discovery}
\begin{algorithmic}
\STATE {\bfseries Input:} demonstrated action trajectory $\iota=(a_1, a_2, ..., a_n)$, routine candidate select number $K$, similarity threshold $\alpha$, length balancing factor $\lambda^{length}$
\STATE Input the first action $a_1$ to create the production $S \rightarrow a_1$
\STATE \textbf{\# Routine Proposal by Sequitur}
\FOR{every action $a_i \in \iota$}
    \STATE Try to match existing rules to generate $(a_1, ..., a_i)$
    \STATE Create a new rule if a new diagram of actions appears and repeats twice
    \STATE Remove a rule if it is used only once
\ENDFOR
\STATE Initialize a collection of routine candidates $\mathcal{C} \leftarrow \emptyset$
\FOR{each introduced non-terminal variable $\rho$}
    \STATE Transfer $\rho$ to a sequence of action primitives by appling the rules
    \STATE Append $\rho$ to $\mathcal{C}$
\ENDFOR

\STATE \textbf{\# Routine Selection}

\STATE Initialize a routine library $\MRDPL \leftarrow \emptyset$
\FOR{each routine candidate $\rho \in \mathcal{C}$}
    \STATE $f(\rho)$ = the frequency of $\rho$ in $\iota$
    \STATE Calculate the score of $\rho$ by $f(\rho) + \lambda^{length} |\rho|$
    \STATE Put $\rho$ into $\MRDPL$
    \IF {there are routines in $\MRDPL$ whose Levenshtein distance is smaller than $\alpha$}
    \STATE Leave one with the highest score
    \ENDIF
\ENDFOR
\STATE Remove routines with lowest scores so that $|\MRDPL| = K$
\STATE \textbf{return} $\MRDPL$

\end{algorithmic}
\end{algorithm}

\begin{figure*}[t]
\centering
\includegraphics[width=1.0\textwidth]{Figure/v1_plot_supple.pdf}
\caption{Ablation study on various hyper-parameters.}
\label{Fig:ablation_parameter}
\end{figure*}

\section{Pseudo-codes}
\label{sec:pseudo_codes}
In Algorithm~\ref{alg:routine_discovery}, we present the procedure of routine discovery from a single demonstration. 

\section{Experimental Details}
\myparagraph{Hyper-parameters} We select hyper-parameters by coarsely running experiments on eight Atari games (the same games used in the main text). For each experiment, we repeat for five agents and report both the mean and standard error in Figure~\ref{Fig:ablation_parameter}. We can observe that RAPL-A2C works well for a wide range of hyper-parameters.

\myparagraph{Implementation} We thank the author of \citet{SQIL} for providing the implementation of BC, GAIL, and SQIL. We adopt the public code under Pytorch to implement A2C \citep{pytorchrl}. The implementation of the ComPILE model \citep{CompILE} originates from its official release, despite that we train the controller via A2C.





==> text/s1_More_Results.tex <==
\section{Additional Experiment Results}
We provide training curves for the imitation learning experiments in Figure~\ref{Fig:curve_imitation_learning}. Moreover, we provide detailed scores for imitation learning on all the Atari games in Table~\ref{tab:numbers_imitation_learning}. We also provide detailed scores for reinforcement learning on all the Atari games in Table~\ref{tab:numbers_reinforcement_learning}.

\begin{figure*}[t]
\begin{center}
\includegraphics[width=1.0\textwidth]{Figure/sqil_plot_atari_v2.pdf}
\vspace{-15pt}
\caption{Training curves on Atari games in comparison with several imitation learning baselines. We plot both the mean and standard deviation in those curves across five agents with random seeds.}
\label{Fig:curve_imitation_learning}
\end{center}
\vspace{-10pt}
\end{figure*}


\begin{table*}[t]
\caption{Results to compare RAPL-SQIL with several imitation learning baselines on Atari games. Each number in the table represents average score and standard over five random seeds. Denote the scores of RAPL-SQIL and human are $S_{R}$ and $S_{H}$ accordingly. The \textbf{Normalized \%} is calculated by $S_{R}/ S_{H} * 100$ \citep{dqn}. The human score of Phoenix is tested by us, which is $6002.0$.}
\label{tab:numbers_imitation_learning}
\centering
\vspace{5pt}
%\setlength{\tabcolsep}{5.5pt}
\begin{tabular}{c|c|c|c|c|c}
\toprule
 & BC & GAIL & SQIL & \textbf{RAPL-SQIL} & \textbf{Normalized \%} \\ \midrule
Freeway & 4.1 $\pm$ 1.2 & 12.4 $\pm$ 2.9 & 5.9 $\pm$ 1.9 & 13.1 $\pm$ 3.7 & 44.3 $\pm$ 1.3 \\
Assault & 523.8 $\pm$ 32.7 & 631.7 $\pm$ 12.3 & 529.1 $\pm$ 30.7 & 677.3 $\pm$ 29.8 & 45.3 $\pm$ 2.0 \\
WizardOfWor & 1239.4 $\pm$ 111.7 & 1980.7 $\pm$ 183.2 & 2140.5 $\pm$ 116.1 & 2212.6 $\pm$ 113.9 & 46.5 $\pm$ 2.4 \\
UpNDown & 1331.3 $\pm$ 12.7 & 1398.1 $\pm$ 17.5 & 3012.3 $\pm$ 21.3 & 428.0 $\pm$ 11.9 & 4.7 $\pm$ 0.0 \\
Amidar & 275.3 $\pm$ 115.9 & 416.9 $\pm$ 124.6 & 441.8 $\pm$ 127.5 & 559.1 $\pm$ 131.1 & 33.4 $\pm$ 7.8 \\
Hero & 321.7 $\pm$ 12.1 & 459.2 $\pm$ 32.8 & 443.6 $\pm$ 49.4 & 639.0 $\pm$ 67.2 & 2.5 $\pm$ 0.1 \\
FishingDerby & 3.1 $\pm$ 1.3 & 0.4 $\pm$ 2.0 & 1.3 $\pm$ 2.0 & 2.4 $\pm$ 0.8 & 43.6 $\pm$ 14.5 \\
Alien & 324.3 $\pm$ 126.8 & 305.6 $\pm$ 154.3 & 523.1 $\pm$ 112.8 & 450.0 $\pm$ 179.1 & 6.5 $\pm$ 2.6 \\
Bowling & 81.5 $\pm$ 8.7 & 129.3 $\pm$ 9.1 & 192.4 $\pm$ 4.6 & 32.1 $\pm$ 3.4 & 20.7 $\pm$ 2.2 \\
BankHeist & 42.1 $\pm$ 2.8 & 104.2 $\pm$ 12.3 & 106.3 $\pm$ 14.2 & 421.1 $\pm$ 28.4 & 57.3 $\pm$ 3.9 \\
Atlantis & 1920.7 $\pm$ 338.1 & 3321.5 $\pm$ 274.9 & 2043.5 $\pm$ 521.7 & 2978.6 $\pm$ 792.2 & 10.3 $\pm$ 0.0 \\
Qbert & 2342.5 $\pm$ 421.3 & 2939.6 $\pm$ 319.8 & 2539.1 $\pm$ 260.4 & 3012.6 $\pm$ 331.4 & 22.4 $\pm$ 2.4 \\
Jamesbond & 42.2 $\pm$ 18.5 & 109.6 $\pm$ 17.2 & 302.7 $\pm$ 21.8 & 375.1 $\pm$ 32.8 & 92.2 $\pm$ 8.0 \\
Asteroids & 241.9 $\pm$ 11.8 & 180.1 $\pm$ 22.7 & 243.6 $\pm$ 44.2 & 260.7 $\pm$ 56.9 & 2.0 $\pm$ 0.0 \\
Kangaroo & 1211.3 $\pm$ 19.4 & 1294.5 $\pm$ 21.8 & 2043.6 $\pm$ 42.8 & 2412.9 $\pm$ 44.3 & 79.5 $\pm$ 1.4 \\
KungFuMaster & 3214.9 $\pm$ 391.7 & 3572.1 $\pm$ 320.8 & 4053.2 $\pm$ 412.4 & 4512.9 $\pm$ 188.2 & 19.8 $\pm$ 0.8 \\
NameThisGame & 1023.2 $\pm$ 314.8 & 2031.3 $\pm$ 422.5 & 2065.7 $\pm$ 191.2 & 2104.7 $\pm$ 59.8 & 51.6 $\pm$ 1.5 \\
CrazyClimber & 3321.6 $\pm$ 222.9 & 1324.9 $\pm$ 533.4 & 4212.2 $\pm$ 121.8 & 4231.7 $\pm$ 317.9 & 12.0 $\pm$ 0.9 \\
MsPacman & 4012.9 $\pm$ 848.7 & 4209.1 $\pm$ 531.9 & 5378.9 $\pm$ 634.5 & 5469.2 $\pm$ 928.6 & 34.9 $\pm$ 5.8 \\
Centipede & 2011.3 $\pm$ 117.2 & 2310.4 $\pm$ 224.1 & 3032.4 $\pm$ 98.0 & 3139.5 $\pm$ 122.3 & 26.2 $\pm$ 1.0 \\
SpaceInvaders & 421.8$\pm$ 41.2 & 590.7 $\pm$ 99.0 & 1232.3 $\pm$ 37.8 & 1420.4 $\pm$ 253.9 & 86.0 $\pm$ 15.3 \\
Tutankham & 42.7 $\pm$ 5.2 & 134.1$\pm$ 6.3 & 203.5 $\pm$ 29.5 & 241.8$\pm$ 25.7 & 144.3 $\pm$ 15.3 \\
ChopperCommand & 201.2 $\pm$ 37.1 & 667.0 $\pm$ 45.9 & 332.3 $\pm$ 49.1 & 720.0 $\pm$ 85.6 & 7.3 $\pm$ 0.9 \\
TimePilot & 592.8 $\pm$ 22.4 & 802.1$\pm$ 33.5 & 1321.3$\pm$ 44.8 & 1349.5$\pm$ 52.0 & 22.8 $\pm$ 0.8 \\
Enduro & 0.0 $\pm$ 0.0 & 3.3 $\pm$ 1.2 & 2.1$\pm$ 1.0 & 13.2 $\pm$ 3.5 & 4.3 $\pm$ 0.0 \\
Gopher & 1231.3$\pm$ 41.8 & 1532.8$\pm$ 53.1 & 1432.5$\pm$ 48.3 & 1952.7$\pm$ 57.9 & 84.1 $\pm$ 2.5 \\
Frostbite & 431.6$\pm$ 52.1 & 512.8$\pm$ 83.1 & 578.6$\pm$ 61.9 & 642.1$\pm$ 72.8 & 14.8 $\pm$ 1.7 \\
Krull & 1391.7$\pm$114.3 & 1785.0$\pm$152.9 & 653.9$\pm$121.4 & 2325.0$\pm$223.8 & 97.1 $\pm$ 9.3 \\
BeamRider & 512.5$\pm$41.2 & 1021.8$\pm$89.6 & 330.3$\pm$42.6 & 1258.9$\pm$251.3 & 21.8 $\pm$ 4.3 \\
Breakout & 3.2$\pm$ 2.1 & 8.1$\pm$1.0 & 5.3$\pm$0.4 & 10.4$\pm$4.1 & 32.7 $\pm$ 0.0 \\
Asterix & 1324.1$\pm$ 122.3 & 2635.0$\pm$ 224.8 & 2178.2$\pm$89.5 & 1210.0$\pm$82.5 & 14.2 $\pm$ 1.0 \\
Phoenix & 504.4$\pm$63.1 & 617.2$\pm$44.8 & 201.9$\pm$64.8 & 391.5$\pm$73.1 & 6.5 $\pm$ 1.2 \\
DemonAttack & 664.8$\pm$ 78.1 & 1794.2$\pm$91.3 & 401.4$\pm$144.8 & 2445.1$\pm$129.4 & 71.9 $\pm$ 3.8 \\ \bottomrule
\end{tabular}
\vskip -0.1in
\end{table*}

\begin{table*}[t]
\caption{Results to compare RAPL-A2C with several reinforcement learning baselines on Atari games. Each number in the table represents average score and standard over five random seeds.}
\label{tab:numbers_reinforcement_learning}
\centering
\vspace{5pt}
%\setlength{\tabcolsep}{5.5pt}
\begin{tabular}{c|c|c|c|c}
\toprule
{} & {ComPILE} & {OptionCritic} & {A2C} & {\textbf{RAPL-A2C}} \\ \midrule
Freeway & 4.2$\pm$2.6 & 11.7$\pm$1.2 & 10$\pm$1.6 & 22.1$\pm$2.4 \\
Assault & 962.1$\pm$37.9 & 1329.7$\pm$304.9 & 2020$\pm$245.4 & 4032$\pm$148.7 \\
WizardOfWor & 687.3$\pm$64.7 & 779.7$\pm$146.1 & 787.2$\pm$34.7 & 1470$\pm$87.2 \\
UpNDown & 14211.7$\pm$2241.7 & 15874.9$\pm$622.9 & 12722.4$\pm$982.1 & 23147.5$\pm$261.8 \\
Amidar & 501.2$\pm$4.4 & 531.7$\pm$6.8 & 132$\pm$3.2 & 231.2$\pm$12.8 \\
Hero & 5964.7$\pm$1001.6 & 6642.6$\pm$287.8 & 9716.1$\pm$459 & 14970.9$\pm$1020.7 \\
FishingDerby & -44.2$\pm$3.6 & -55.2$\pm$0.7 & -66$\pm$0.7 & -33.5$\pm$0.3 \\
Alien & 444.2$\pm$19.1 & 769.4$\pm$26.7 & 721.3$\pm$44.8 & 1067.8$\pm$42.5 \\
Bowling & 13.4$\pm$2.9 & 21.6$\pm$2.1 & 24$\pm$0.7 & 34$\pm$1.5 \\
BankHeist & 643.8$\pm$71.4 & 883.5$\pm$29.8 & 584.6$\pm$36.4 & 822.1$\pm$2.7 \\
Atlantis & 129930.5$\pm$24009.6 & 224449.3$\pm$8131.6 & 197997.2$\pm$3370.6 & 269010.1$\pm$1660.2 \\
Qbert & 6729.4$\pm$1200 & 7864.1$\pm$475.8 & 12942.5$\pm$1646.2 & 16527.4$\pm$261.8 \\
Jamesbond & 134.5$\pm$19.9 & 122.3$\pm$1.6 & 199$\pm$20.7 & 263.7$\pm$24.3 \\
Asteroids & 735.1$\pm$178.3 & 2412.9$\pm$62.2 & 1535.4$\pm$88.4 & 2560.2$\pm$8.6 \\
Kangaroo & 149.6$\pm$26.3 & 220.5$\pm$19 & 221.8$\pm$2.5 & 290$\pm$0.2 \\
KungFuMaster & 12049.4$\pm$406.1 & 28741.2$\pm$467.7 & 24939$\pm$4297.5 & 47218.8$\pm$1775.8 \\
NameThisGame & 3305.3$\pm$162.7 & 4621.8$\pm$498.2 & 4073.8$\pm$375.5 & 5262.6$\pm$156.2 \\
CrazyClimber & 64319.3$\pm$6147.1 & 55691.4$\pm$10913.6 & 88588.6$\pm$8677.5 & 113559.3$\pm$10043.1 \\
MsPacman & 1895$\pm$388.5 & 1886.5$\pm$260 & 2733.5$\pm$198.2 & 4422$\pm$62.4 \\
Centipede & 1322.6$\pm$142.4 & 2682.4$\pm$11.1 & 2542.6$\pm$129.2 & 3132$\pm$206.8 \\
SpaceInvaders & 1894.6$\pm$79.6 & 2583.9$\pm$349.2 & 3312.8$\pm$205.3 & 4592$\pm$269.7 \\
Tutankham & 532.3$\pm$33.3 & 512.5$\pm$123 & 779.4$\pm$79.1 & 1422.5$\pm$32.7 \\
ChopperCommand & 443.1$\pm$36.6 & 532.5$\pm$41.9 & 888.6$\pm$54.4 & 911.9$\pm$66.5 \\
TimePilot & 1354.9$\pm$16.5 & 3442.6$\pm$163.6 & 3453.6$\pm$289.5 & 3490.7$\pm$9.1 \\
Enduro & 0$\pm$0.6 & 0$\pm$0.8 & 1.9$\pm$0.1 & 1.8$\pm$0.7 \\
Gopher & 644.2$\pm$17.3 & 553.6$\pm$73.7 & 966$\pm$64.8 & 928.1$\pm$19.3 \\
Frostbite & 44.2$\pm$22.5 & 236.8$\pm$18.3 & 256.3$\pm$2.8 & 248$\pm$15.4 \\
Krull & 5590.9$\pm$554.9 & 6689.7$\pm$437 & 6791.3$\pm$565.4 & 6041.7$\pm$166.8 \\
BeamRider & 2124.1$\pm$121.5 & 552.1$\pm$130.1 & 2191.2$\pm$100.4 & 1745.4$\pm$67.3 \\
Breakout & 62.7$\pm$10.9 & 144.2$\pm$7.9 & 182.9$\pm$7.5 & 139.8$\pm$7.9 \\
Asterix & 3153.1$\pm$150.8 & 1235.8$\pm$76 & 2463.1$\pm$140.7 & 1823.9$\pm$92.6 \\
Phoenix & 5521.3$\pm$112.9 & 6642.9$\pm$274.1 & 6742.5$\pm$467.3 & 5009$\pm$158 \\
DemonAttack & 3352.1$\pm$207 & 5546.8$\pm$274.7 & 5957.6$\pm$214.4 & 4121$\pm$93.9 \\ \bottomrule
\end{tabular}
\vskip -0.1in
\end{table*}

==> text/s2_Additional_exps.tex <==

\section{Additional Ablation Study}
\subsection{Effect of Parameters in Routine Abstraction}
\label{sec:ablation_paras}
We validate the effectiveness of the parameters used in routine abstraction: the balancing factor $\lambda$, the similarity threshold $n$ and the number of routines $k$. We denote the default parameters (presented in Sec \ref{sec: hyperparameters}) as $\lambda_d$, $n_d$, and $k_d$. For each parameter, we change into different values while other parameters are set to the default values. 

As in other ablation studies in our paper, we train the routine policy via PPO on CoinRun's hard levels. The number of training levels is unbounded while we restrict a training budget of 50k episodes. We report the mean reward of the last 100 episodes. Each experiment is averaged for three seeds.

We show abstracted routine libraries for different parameters in Table \ref{tb:routine_libraries}. Note we only show routines that are not primitive actions. The qualitative results are shown in Figure \ref{Fig:ablation_paras}. We analyze the results in the following paragraphs.

\subsubsection{Balancing Factor} 
A smaller balancing factor indicates a weaker effect of the lengths of routines. When the balancing factor is very small ($\lambda=0.1 \lambda_d)$, the abstracted routines are very short such as \texttt{[RIGHT, RIGHT, RIGHT]}. These routines are ineffective because they are too short to carry enough information as skills. Besides, selecting routines mainly according to the routine length (when $\lambda=100\lambda_d$) is also ineffective because these routines are rarely used.

\subsubsection{Similarity Threshold}
Preventing adding too similar routines is also important. When $n$ is very small, there are too many similar routines in one routine library. Such routines have similar functions and would slow down exploration. On the other hand, when $n$ is very large, too many routines would be pruned. So the abstracted routines are not the ones with best scores. Therefore, a moderate $n$ leads to the best performance.

\subsubsection{Selected Number of Routines}
The number of adopted routines also influences the performance of the training process. Although selecting only one routine can increase the solved levels, abstracting a few more routines can have stronger performance. A too-large routine library would harm performance because a large action space would lead to inefficient exploration.

\subsection{Effect of Adopting the Minimal Action Space on CoinRun}
\label{Sec:minimum action space}
On CoinRun, for the sake of clear presentation, we adopt the minimal action space and remove all the predefined combos (e.g., \texttt{RIGHTDOWN}). Note that the baselines also use the minimal action space in previous experiments on CoinRun. Figure \ref{Fig:ablation_action_space} shows the training curves of routine policies based on full action space and minimum action space. Our routine abstraction and routine policy training algorithm can work even better when adopting the full action space.

\begin{figure}[t]
\vskip 0.2in
\begin{center}
\centerline{
\subfig\includegraphics[width=0.9\columnwidth]{Figure/facoinrun_v1.png}}
\caption{Compare routine policies based on full action space and minimum action space. Although training on full action space has stronger performance, for the sake of better interpretation, we adopt the minimum action space on CoinRun. Refer to Sec \ref{Sec:minimum action space} for more details.}
\label{Fig:ablation_action_space}
\end{center}
\vskip -0.2in
\end{figure}

==> text/s5_Extended_review.tex <==
\section{Extended Review}
\paragraph{Macro-actions} Macro-actions are temporally extended actions that are widely studied in various domains. Sutton \citep{MacroEmpiricalAnalysis1998, SuttonSMDP} refers macro-actions 
(or called \textit{options}) to policies with termination conditions. He has empirically justified that the macro actions can sometimes boost exploration and value propagation. However, in the STRIPS system \citep{STRIPS}, a macro action is a sequence of pre-defined operators that contribute to problem-solving. \citet{1985MacroOperators} instead uses the notion of \textit{macro-operators} built upon primitive operators to efficiently solve problems. In our work, we specify a \textit{routine} to be a sequence of primitive actions, which can be regarded as one specific case of macro actions.

\paragraph{Macro-action Discovery} In the field of theorem proving, MACLEARN \citep{1989Heuristic} conducts searching to find new macros so that the problems can be solved faster or more economically. Besides, Macro-FF \citep{MacroFF} improves AI planning by abstracting macro actions from the problem's domain structure. The abstraction is achieved by a clustering procedure over the problem's graph. These methods are not designed for general MDPs. \citet{OptionsLearning} proposes to learn macro actions by finding frequently visited states. Their method is only suitable for environments with low-level states such as the grid world. \citet{LearnMacroActions1999} implicitly learns macro actions by modeling the transition from one action to another. \citet{yoshikawa2006AcquiringMacroActions} proposes to acquire macro-actions with tree structures in Reinforcement Learning. They assume that the states are discrete (e.g., in a maze); thus, their methods cannot generalize to high-dimension tasks. \citet{DeepRLWithMacroActions} proposes to abstract macro actions during the learning of an RL agent. However, as indicated by their experiments, the frequently changed action space would make the training unstable. The concurrent work \citet{ConstructionMacroActions} utilizes a genetic algorithm to construct macro actions for deep reinforcement learning. Nevertheless, their methods require training RL agents multiple times to find a set of good macro actions, which is very time-consuming.


==> text/s_deprecated.tex <==
\footnote{Although one can sample multiple $N-step$ experiences from the routine experiences, for implementation convenience we only sample one.} 
% \textbf{Right:} visualization of trained agents utilizing abstracted routines on Atari. Each row corresponds to one routine. Every agent is marked by a red circle. (\textbf{top}) In Krull, our agent learns to utilize the routine to jump over the thin white threads of the web (marked via a red arrow). (\textbf{middle}) In Qbert, the agent needs to step on every square to change the color of each one from yellow to blue. It uses one routine to jump down repeatedly, and such a regularized move can help earn a sequence of scores. (\textbf{down}) In Enduro, the agent needs to drive a white car to pass other cars without colliding with them. The \texttt{Fire} operation can increase the speed of the car in Enduro. The abstracted routine helps the agent to pass the racer in the front by moving left and moving forward, which earns more scores. Those abstracted routines contribute to a more interpretable policy.
% We visualize the trained agents with learned routines in Figure \ref{Fig:VisAbstractedRoutinesAtari}. Those abstracted routines are interpretable and produce several advantages. First, they may help the agent overcome obstacles such as the web in Krull. Since exploring by those abstracted skills can easily earn a high score in comparison to exploring by primitive actions, the agent has more possibilities to explore a better policy. Besides, the agent's move can be regularized and smoothed by adopting routines.

% moved to supplementary
% \subsubsection{Implementation Details}
% \myparagraph{Demonstration Collection} For all the games, we generate ten demonstrations via A2C, where each demonstration records one episode before selecting one best demonstration with the highest score as the final demonstration. The selected demonstration is used for both routine discovery and imitation learning.

% \myparagraph{Routine Discovery} In all experiments, we set the balancing factor between frequency and length to be $\lambda=0.1$. Moreover, the number of routines is set to $K=3$, which is validated in the ablation study. Besides, we would leave the best routine between routines whose Levenshtein distance is smaller than $2$.

% \myparagraph{Policy Training} For A2C, we adopt the public code under Pytorch \citep{pytorchrl}. All the network architectures and unspecified hyperparameters are the same as the corresponding baselines to ensure fair comparison. We thank the author of \citet{SQIL} to provide the implementation of BC, GAIL and SQIL. The implementation of ComPILE originates from its official release.

% We compare the full approach to following ablated models:

% \myparagraph{Random Routines (RR)} This validates whether our abstracted routines leverages the information in the demonstration. Let $\MRDPL$ be the library abstracted by our full approach. We create a random routine library $\MRDPL_{r}$ by the following procedure: for each routine $\rho \in \MRDPL$, we create a random routine with the same length as $\rho$ and put it to $\MRDPL_{r}$.

% \myparagraph{Proposal by Enumeration (PbE)} This experiment is designed to examine whether the Sequitur can discover good routine candidates from the demonstration. We enumerate all the possible combinations of primitive actions to form routine candidates. Note that there are infinite possible routines when their lengths are not restricted. We set the maximum length of enumerated routines to be the longest routine of the routine library discovered by Sequitur.

% \myparagraph{Without Length Metric (WLM)} This experiment measures whether we should encourage the longer routines to be selected. Specifically, we set $\lambda=0$ in Equation \ref{eq:rtscore} to sorely measure routines by their frequencies. This model is most similar to \cite{LearningPlan1972}.

% \myparagraph{Without Similarity Restriction (WSR)} Recall that in Algorithm \ref{alg:routine_evaluation}, we restrict the similarity of two routines to be at most $n$. We remove this restriction in this ablated version.

% Despite the specified ablated component, other details are the same as the full model presented in Sec \ref{sec: approach}. We train each model on unbounded hard levels via PPO with a limited budget of 50k episodes. To alleviate the randomness, we run each model for three times and report both the mean and standard deviation in Figure \ref{Fig:AblationResults}. We observe that ablating any of the components would harm the performance of discovered routines. Although Proposal by Enumeration could achieve nearly the same performance as the full model, it is over 100 times slower than the full model to finish the routine abstraction. Random routines perform worst among all the models because it does not leverage the information of demonstration and only randomly combine primitive actions. The inferior performance of WLM and WSR implies that it is better to promote relatively longer and unique routines. 

% \begin{algorithm}[htb]
%   \caption{RoutineProposal}
%   \label{alg:propose_by_sequitur}
% \begin{algorithmic}
% \STATE {\bfseries Input:} action trajectory $\iota=(a_1, a_2, ..., a_n)$
% \STATE Input the first action $a_1$ to create the production $S \rightarrow a_1$
% \STATE \textbf{\# Discover grammar structure by Sequitur}
% \FOR{every action $a_i \in \iota$}
%     \STATE Try to match existing rules to generate $(a_1, ..., a_i)$
%     \STATE Create a new rule if a new diagram of actions appears and repeats twice
%     \STATE Remove a rule if it is used only once
% \ENDFOR
% \STATE \textbf{\# Transfer non-terminal variables to routines}
% \STATE Initialize a collection of routine candidates $\mathcal{C} \leftarrow \emptyset$
% \FOR{each introduced non-terminal variable $\rho$}
%     \STATE Transfer $\rho$ to a sequence of action primitives
%     \STATE Append $\rho$ to $\mathcal{C}$
% \ENDFOR
% \STATE \textbf{return} $\mathcal{C}$
% \end{algorithmic}
% \end{algorithm}
% \subsubsection{Routine Proposal}
% \label{subsec:RoutineProposal}


% \begin{algorithm}[htb]
%   \caption{RoutineEvaluation}
%   \label{alg:routine_evaluation}
% \begin{algorithmic}
% \STATE {\bfseries Input:} proposed routine candidates $\mathcal{C}$, action trajectory $\iota$, routine candidate select number $k$, similarity threshold $n$
% \STATE Initialize a routine library $\MRDPL \leftarrow \emptyset$
% \FOR{each routine candidate $\rho \in \mathcal{C}$}
%     \STATE Calculate the score of $\rho$ by Equation \ref{eq:rtscore}
%     \STATE Put $\rho$ into $\MRDPL$
%     \IF {there are two routines in $\MRDPL$ whose Levenshtein distance is smaller than $n$}
%     \STATE Leave one with the highest score
%     \ENDIF
%     \IF {$\| \MRDPL \| > k$}
%     \STATE Remove one routine in $\MRDPL$ with the lowest score
%     \ENDIF
% \ENDFOR
% \STATE Put all primitive actions into $\MRDPL$
% \STATE \textbf{return} $\MRDPL$
% \end{algorithmic}
% \end{algorithm}



% IS
% (actually there is no mask in the implementation, so no IS is used.) Because the routine is temporally composed of the primitive actions, the transition of executing a routine also can be viewed as the successive transitions of executing several primitive actions in order. For a routine  $\rho_{t}=(a_{t}, a_{t+1}, ..., a_{t+k-1})$, the corresponding policy gradient for the primitive action $a_{t}$ can be estimated via importance sampling (IS) correction $\mathbb{E}_{a_{t}~\sim\pi^{'}(.|s_{t})}\Big[ A(s_{t}) \nabla_{\theta}\log(\pi^{'}(a_{t} | s_{t}, \theta)) \Big] = \mathbb{E}_{\rho_{t}~\sim\pi(.|s_{t})}\Big[ \frac{\pi^{'}(a_{t} | s_{t})}{\pi(\rho_{a} | s_{t})} A(s_{t})  \nabla_{\theta} \log(\pi^{'}(a_{t} | s_{t}, \theta)) \Big]$. Similarly the policy gradients of the following actions can be derived via IS correction. The importance sampling ratio $\frac{\pi(a_{t} | s_{t})}{\pi(\rho_{a} | s_{t})}$ may cause high variance of the gradients, so we clip the ratio $\ceil*{\frac{\pi(a_{t} | s_{t})}{\pi(\rho_{a} | s_{t})}}$ and discard transitions with small $\pi(a_{t}|s_{t},\theta)$ in practice. The combined policy gradient for the augmented action space is thus  $\mathbb{E}_{\rho_{t}~\sim\pi(.|s_{t})}\Big[ A(s_{t}) \nabla_{\theta} \log(\pi(\rho_{t} | s_{t}, \theta)) + \ceil*{\frac{\pi(a_{t} | s_{t})}{\pi(\rho_{a} | s_{t})}} A(s_{t})  \nabla_{\theta} \log(\pi(a_{t} | s_{t}, \theta)) \Big]$. 
% similar extension for off-policy value based reinforcement learning methods such as DQN or Rainbow. 
